MagicAnimate: Temporally Consistent Human Image Animation using Diffusion Model

This paper studies the human image animation task, which aims to generate a video of a certain reference identity following a particular motion sequence. Existing animation works typically employ the frame-warping technique to animate the reference image towards the target motion. Despite achieving reasonable results, these approaches face challenges in maintaining temporal consistency throughout the animation due to the lack of temporal modeling and poor preservation of reference identity. In this work, we introduce MagicAnimate, a diffusion-based framework that aims at enhancing temporal consistency, preserving reference image faithfully, and improving animation fidelity. To achieve this, we first develop a video diffusion model to encode temporal information. Second, to maintain the appearance coherence across frames, we introduce a novel appearance encoder to retain the intricate details of the reference image. Leveraging these two innovations, we further employ a simple video fusion technique to encourage smooth transitions for long video animation. Empirical results demonstrate the superiority of our method over baseline approaches on two benchmarks. Notably, our approach outperforms the strongest baseline by over 38% in terms of video fidelity on the challenging TikTok dancing dataset. Code and model will be made available.

==> sec/5_limitations.tex <==
\section{Limitations}
\ours{} achieves state-of-the-art human image animation results and demonstrates strong robustness for unseen data. However, there is still room for improvement in several aspects: (1) Although DensePose provides a dense guidance for the animation, there exists flickering and occasional failures for the DensePose estimation method~\cite{wu2019detectron2}. Therefore, enhancing the robustness and accuracy of the DensePose estimator would contribute to the overall performance of our human animation. (2) Densepose also lacks control signals for the facial and finger details. Addressing this gap by incorporating a multi-ControlNet approach could potentially enhance the control ability for faces and hands, leading to more realistic and detailed animations. (3) While diffusion-based methods offer high-quality results, they are generally less efficient than GAN-based methods due to multiple denoising sampling steps. Exploring strategies to improve the efficiency of \ours{} could enhance its applicability.
